RAGO: Recurrent Graph Optimizer For Multiple Rotation Averaging

This paper proposes a deep recurrent Rotation Averaging Graph Optimizer (RAGO) for Multiple Rotation Averaging (MRA). Conventional optimization-based methods usually fail to produce accurate results due to corrupted and noisy relative measurements. Recent learning-based approaches regard MRA as a regression problem, while these methods are sensitive to initialization due to the gauge freedom problem. To handle these problems, we propose a learnable iterative graph optimizer minimizing a gauge-invariant cost function with an edge rectification strategy to mitigate the effect of inaccurate measurements. Our graph optimizer iteratively refines the global camera rotations by minimizing each node's single rotation objective function. Besides, our approach iteratively rectifies relative rotations to make them more consistent with the current camera orientations and observed relative rotations. Furthermore, we employ a gated recurrent unit to improve the result by tracing the temporal information of the cost graph. Our framework is a real-time learning-to-optimize rotation averaging graph optimizer with a tiny size deployed for real-world applications. RAGO outperforms previous traditional and deep methods on real-world and synthetic datasets. The code is available at https://github.com/sfu-gruvi-3dv/RAGO

==> equations/camera_random_init.tex <==
\begin{equation}
\mathbf{q}^{init}_{i} = \text()
\label{eq:edge_conv_equ}
\end{equation}

==> equations/cost_map_to_feature.tex <==
\begin{equation}
    \{C_{u}^{t}\}, \{C_{uv}^{t}\} = \Theta_{\text{cost}}(\{d_{u}^{t}\}, \{d_{uv}^{t}\},\mathcal{G})
\end{equation}

==> equations/evaluation_cost.tex <==
% \begin{equation}
%  \{\hat{\mathbf{R}}_{u}\} = \mathop{\arg\min}_{ \{\tilde{\mathbf{R}}^{t}_{u}\} } \sum_{(u,v)\in \mathcal{E}}\rho(d(\check{\mathbf{R}}_{uv},\mathbf{R}_{uv}))^2d(\tilde{\mathbf{R}}_{uv}, \mathbf{R}_{uv})
%   \label{eq:eval_cost}
% \end{equation}
\begin{equation}
\sum_{(u,v)\in \mathcal{E}}\rho(d(\mathbf{R}_{uv}^t,\mathbf{R}_{uv}))^2d(\mathbf{R}^{t}_{u}\mathbf{R}_{v}^{t\top}, \mathbf{R}_{uv}),
  \label{eq:eval_cost}
\end{equation}

==> equations/gauge_freedom.tex <==
\begin{equation}
    \mathbf{R}_{uv} = \mathbf{R}_{u}\mathbf{R}^{-1}_{v} = (\mathbf{R}_{u}\mathbf{R})(\mathbf{R}_{v}\mathbf{R})^{-1}, \forall \mathbf{R} \in SO(3)
\end{equation}

==> equations/gru_equ.tex <==
\begin{equation}
\begin{split}
    \mathbf{z}^{t} &= \sigma(\Phi_{z}([\mathbf{h}^{t-1},\mathbf{I}^{t}])), \\
    \mathbf{r}^{t} &= \sigma(\Phi_{r}([\mathbf{h}^{t-1},\mathbf{I}^{t}])), \\
    \tilde{\mathbf{h}}^{t} &= \text{tanh}(\Phi_{\mathbf{h}}([\mathbf{r}^{t}\odot \mathbf{h}^{t-1},\mathbf{I}^{t}])),\\
    \mathbf{h}^{t} &= (\mathbf{1}-\mathbf{z}^{t})\odot \mathbf{h}^{t-1} + \mathbf{z}^{t}\odot \tilde{\mathbf{h}}^{t}.
\end{split}
\label{eq:gru_equ}
\end{equation}

==> equations/model_eval.tex <==
\begin{equation}
 \{\reallywidebar{\mathbf{R}}_{i}^{*}\} = \mathop{\arg\min}_{\{ \mathbf{R}^*_i\}}\sum_{(i,j) \in \mathcal{E}}{\rho(d(\widetilde{\mathbf{R}}_{ij}, \mathbf{R}^*_j{\mathbf{R}_i^{*}}^{-1})},
  \label{eq:model_cost}
\end{equation}

==> equations/mra_cost_func.tex <==
\begin{equation}
    d(\{\mathbf{R}_u\}) = \sum_{(u,v)\in E}distance(\mathbf{R}_{uv}, \mathbf{R}_{u}\mathbf{R}_{v}^{-1})^{p}
\end{equation}

==> equations/rotation_optimized.tex <==
\begin{equation}
\bar{\mathbf{R}}_{u} \leftarrow \tilde{\mathbf{R}}^{t}_{u},\; \; \; \bar{\mathbf{R}}_{uv} \leftarrow \check{\mathbf{R}}^{t}_{uv}
\end{equation}

==> equations/sra_objective.tex <==
%\begin{equation}
% \{\reallywidebar{\mathbf{R}}_{i}^{*}\} = \mathop{\arg\min}_{\{ \mathbf{R}^*_i\}}\sum_{(i,j) \in \mathcal{E}}{\rho(d(\widetilde{\mathbf{R}}_{ij}, \mathbf{R}^*_j{\mathbf{R}_i^{*}}^{-1})},
%  \label{eq:mra_objective}
%\end{equation}
\begin{equation}
    \mathbf{R}^{*} = \arg\min_{\mathbf{R}} \sum_{i=1}^{n}d(\mathbf{R}_i, \mathbf{R}) 
    \label{eq:sra_objective}
\end{equation}

==> equations/train_init_loss.tex <==
\begin{equation}
    \mathit{L}_{\text{init}} = \frac{1}{|\mathcal{E}|}\sum_{(i,j)\in \mathcal{E}} L_{\text{BCE}}(w_{ij}, y_{ij})
    \label{eq:loss_init}
\end{equation}

==> equations/train_total_loss.tex <==
\begin{equation}
    \mathit{L}_{\text{total}} = \mathit{L}_{\text{init}} + \mathit{L}_{\text{opt}}
    \label{eq:loss_total}
\end{equation}

==> equations/update_pred.tex <==
\begin{equation}
    \Delta R^{t} = \Phi(h^{t})
\end{equation}

==> figures/edge_conv.tex <==
\begin{figure}[t]
	\centering
	\scriptsize
	\includegraphics[width=\linewidth]{figures/edge_conv_img.pdf}
	%\vspace{2cm}
	\caption{Alternative iteration. RAGO first refines the relative orientations for $t_e$ times, and then optimizes the estimated camera orientations for $t_n$ times. The orientations on edges and nodes will iterative $t_e\times t_g$ and $t_n\times t_g$ times in total, respectively.}
	\label{fig:edge_conv}
    \vspace{-1em}
\end{figure}

==> figures/edge_conv_2.tex <==
\begin{figure}[t]
	\centering
	\scriptsize
	\includegraphics[width=\linewidth]{figures/edge_conv_2_img.pdf}
	%\vspace{2cm}
	\caption{The structure of an Edge Convolution. An Edge Convolution update each edge feature with a weight shared MLP $\Phi_{\text{edge}}$. Then, the node features are updated by passing the updated edge features from the neighbors to the node MLP $\Phi_{\text{node}}$. }
	\label{fig:edge_conv_2}
    \vspace{-1em}
\end{figure}

==> figures/edge_conv_3.tex <==
\begin{figure}[t]
	\centering
	\scriptsize
	\includegraphics[width=\linewidth]{figures/edge_conv_3_img.pdf}
	%\vspace{2cm}
	\caption{The structure of edge convolution. An edge convolution update each edge feature with a shared weight MLP $\Phi_{\text{edge}}$. Then, the node features are updated by passing the aggregation feature from the neighbors to the node MLP $\Phi_{\text{node}}$. }
	\label{fig:edge_conv_3}
    \vspace{-1em}
\end{figure}

==> figures/pipeline.tex <==
\begin{figure*}[ht]
	\centering
	\scriptsize
	\includegraphics[width=\textwidth]{figures/pipeline_img.pdf}
	%\vspace{2cm}
	\caption{The pipeline of our method. Gevin a set of observed relative orientations $\{\mathbf{R}_{ij}\}$, the initial guess of global orientations $\{\mathbf{R}_{i}\}$ is computed by the random or GCO initializer. The view-graph is first fed to an MPNN for feature extraction and hidden states initialization. For iterative optimization, we first compute the SRA cost graph $\{C^{t}\}$ from the current estimated global orientation $\{\tilde{\mathbf{R}}^{t}_{i}\}$ and rectified relative orientations $\{\check{\mathbf{R}}^{t}_{ij}\}$. The graph updater then computes incremental solution of orientations $\{\Delta\mathbf{R}^{t}\}$ to update $\{\tilde{\mathbf{R}}^{t}_{i}\}$ and $\{\check{\mathbf{R}}^{t}_{ij}\}$. Finally, the global absolute orientations gradually converge to the optimum, $\{\hat{\mathbf{R}}_{i}\}$}
	\label{fig:pipeline}
    \vspace{-1em}
\end{figure*}

==> figures/pipeline_v2.tex <==
\begin{figure*}[ht]
	\centering
	\scriptsize
	\includegraphics[width=\textwidth]{figures/pipeline_v2_img.pdf}
	%\vspace{2cm}
	\caption{The pipeline of our Rotation Averaging Graph Optimizer (RAGO). We use Message Passing Neural Network (MPNN) $\Theta$ ~\cite{MPNN} to extract feature from the input graph. (a) Camera Orientation Initialization: The initial global orientations $\{\mathbf{R}_{u}\}$ are generated randomly or by other methods. (b) Feature Extraction and Hidden State Initialization: The view-graph is first fed to two (MPNN) $\Theta_{\text{feat}}$ and $\Theta_{\text{state}}$ for feature extraction and hidden states initialization. (c) Iterative Optimization \heng{i change it to light blue but it becomes 
uglier}\ping{the background color of this part is ugly and very similar to that of (b). Make it more different, use light blue/green}: For iterative optimization, we first compute the SRA cost graph $\{d^{t}\}$ from $\{\mathbf{R}^t\}$. Then a MPNN $\Theta_{\text{cost}}$ extract cost feature $\{C^t\}$ from $\{d^t\}$. The graph updater generates $\{I^t\}$ by concatenating $\{\mathbf{R}^t\}$, $\{f\}$ and $\{C^t\}$. A GRU module takes ${I^t}$ to update the hidden state $\{h^t\}$, then computes incremental update of orientations $\{\Delta\mathbf{R}^{t}\}$ to update $\{\tilde{\mathbf{R}}^{t}_{u}\}$ and $\{\check{\mathbf{R}}^{t}_{uv}\}$. Please refer to the main text for specific details. \ping{this caption is too long. Simplify it and refer to the text in the paper for details.}}
	\label{fig:pipeline}
    \vspace{-1em}
\end{figure*}

==> main/3_1_architecture.tex <==
% arch

==> main/temp.tex <==
%temp

==> table/1dsfm_table_2021.tex <==
\begin{table*}[h!t]
\begin{center}
\scalebox{0.85}{
\begin{tabular}{ccl|cc|cc|cc|cc|cc}
\hline
\multicolumn{3}{c|}{Datasets} & \multicolumn{2}{c|}{Chatterjee\cite{ICCV2013}} & \multicolumn{2}{c|}{Arrigoni\cite{Arrigoni2018RobustSI}}& \multicolumn{2}{c|}{NeuRoRA\cite{ECCV2020_neurora}} & \multicolumn{2}{c|}{MPLS\cite{Shi2020MessagePL}}& \multicolumn{2}{c}{Ours} \\
\hline \hline
\#image & \#edge & Names & mn    & md    & mn    & md  & mn    & md  & mn   & md   & mn   & md   \\ 
                  577  & 59.5\%  & Alamo               & 4.2  & \textbf{1.1}  &6.2 &1.6 & 4.94          & 1.16          & 3.44                 & 1.16                 & \textbf{2.89}                      & \textbf{1.07}                  \\
    227  & 66.8\%  & Ellis Island       & 2.8  & \textbf{0.5}& 3.9  & 1.2 & 2.59          & 0.64 & 2.61                 & 0.88                 & \textbf{1.88}                     & 0.83                 \\
677  & 17.5\% & Gendarmenmarkt  & 37.6 & 7.7 & 41.6 & 13.3 & \textbf{4.51}          & \textbf{2.94}          & 44.9                 & 8.0                    & 6.29  & 3.69  \\
341  & 30.7\%  & Madrid Metropolis              & 6.9  & 1.2 & 6.0  & 1.7 & \textbf{2.55} & 1.13          & 4.65                 & 1.26                 & 2.96                              & \textbf{1.09}        \\
450  & 46.8\%  & Montreal Notre Dame & 1.5  & \textbf{0.5}& 4.8  & 0.9 & 1.2           & 0.6           & 1.04        & 0.51        & \textbf{0.91}                     & \textbf{0.5}         \\
338  & 39.5\%  & Piazza del Popolo   & 4    & 0.8& 10.8    & 1.2 & 3.05          & 0.79          & 3.73                 & 1.93                 & \textbf{2.68}                     & \textbf{0.76}        \\
  1084 & 10.9\%  & Roman Forum         & 3.1  & 1.5 & 13.2  & 8.2 & 2.39          & 1.31          & 2.62                 & 1.37                 & \textbf{2.04}                     & \textbf{1.19}        \\
472  & 18.5\%  & Tower of London        & 3.9  & 2.4& 4.6  & 1.8 & 2.63          & 1.46          & 3.16                 & 2.2                  & \textbf{2.55}                     & \textbf{1.25}        \\
5058 & 4.6\%   & Trafalgar           & 3.5  & 2 & 48.6  & 13.2   & 5.33          & 2.25          &  \multicolumn{2}{c|}{-} & \multicolumn{2}{c}{\footnotesize{Out of Memory}} \\ 
789  & 5.9\%   & Union Square       & 9.3  & 3.9 & 9.2  & 4.4 & 5.98          & 2.01          & 6.54                 & 3.48                 & \textbf{4.37}                     & \textbf{1.85}        \\
836  & 24.6\%  & Vienna Cathedral    & 8.2  & 1.2& 19.3  & 2.39 & \textbf{3.9}  & 1.5           & 7.21                 & 2.83                 & 3.91                              & \textbf{1.1}         \\
437  & 26.5\%  & Yorkminster         & 3.5  & 1.6& 4.5  & 1.6 & 2.52          & 0.99          & 2.47                 & 1.45                 & \textbf{2.27}                     & \textbf{0.91}        \\
2152 & 10.2\%  & Piccadilly          & 6.9  & 2.9& 22.0  & 9.7 & 4.75          & 1.91          & 3.93                 & 1.81                 & \textbf{3.63}                     & \textbf{1.8}         \\
332  & 29.3\% & NYC Library        & 3    & 1.3   & 3.9    & 1.5 & 1.9           & 1.18          & 2.63                 & 1.24                 & \textbf{1.75}                     & \textbf{1.12}  \\
\hline    
% \multicolumn{13}{c}{mn: mean of the angular error (in deg); md: median of the angular error (in deg);}                      \\
\end{tabular}
}
\end{center}
\vspace{-0.5em}
\caption{Comparison of results on the \textit{\textbf{1DSfM}} dataset. We compare our method with various SOTA MRA methods. Mean(mn) and median(md) angular errors on the estimated absolute rotations are compared. The entries with the best performance are bolded.}
\label{table:1dsfm_table}
% \vspace{-1em}
\end{table*}

==> table/__latexindent_temp.tex <==
% \begin{table*}[h!t]
% \begin{center}
% \scalebox{0.85}{
% \begin{tabular}{ccl|cc|cc|cc|cc|cc|cc}
% \hline
% \multicolumn{3}{c|}{Setting} & \multicolumn{2}{c|}{$t=1$} & \multicolumn{2}{c|}{$t=5$}& \multicolumn{2}{c|}{$t=20$} & \multicolumn{2}{c|}{$t=100$}& \multicolumn{2}{c|}{Avg. Time}& \multicolumn{2}{c}{CVPR2021} \\
% \hline \hline
% \#image & \#edge & Names & mn    & md    & mn    & md  & mn    & md  & mn   & md   & mn   & md& mn   & md   \\ 
%                   577  & 59.5\%  & Alamo               & 4.2  & 1.1  &6.2 &1.6 & 4.94          & 1.16          & 3.44                 & 1.16      & 2.82      &   0.88          & 2.89                      & 1.07                  \\
%     227  & 66.8\%  & Ellis Island       & 2.8  & 0.5& 3.9  & 1.2 & 2.59          & 0.64 & 2.61                 & 0.88           & 1.74&  0.46     & 1.88                   & 0.83                 \\
% 677  & 17.5\% & Gendarmenmarkt  & 37.6 & 7.7 & 41.6 & 13.3 & 4.51          & 2.94          & 44.9                 & 8.0     & 5.24 &     2.68           & 6.29  & 3.69  \\
% 341  & 30.7\%  & Madrid Metropolis              & 6.9  & 1.2 & 6.0  & 1.7 & 2.55 & 1.13          & 4.65                 & 1.26  &    3.05& 1.03               & 2.96                              & 1.09        \\
% 450  & 46.8\%  & Montreal Notre Dame & 1.5  & 0.5& 4.8  & 0.9 & 1.2           & 0.6           & 1.04        & 0.51       &0.86&0.46       & 0.91           & 0.5         \\
% 338  & 39.5\%  & Piazza del Popolo   & 4    & 0.8& 10.8    & 1.2 & 3.05          & 0.79          & 3.73                 & 1.93        &1.91&0.63         & 2.68                   & 0.76        \\
%   1084 & 10.9\%  & Roman Forum         & 3.1  & 1.5 & 13.2  & 8.2 & 2.39          & 1.31          & 2.62                 & 1.37     &2.55& 1.10           & 2.04                     & 1.19        \\
% 472  & 18.5\%  & Tower of London        & 3.9  & 2.4& 4.6  & 1.8 & 2.63          & 1.46          & 3.16                 & 2.2        &2.51&1.20          & 2.55                     & 1.25        \\
% 5058 & 4.6\%   & Trafalgar           & 3.5  & 2 & 48.6  & 13.2   & 5.33          & 2.25          &  \multicolumn{2}{c|}{-} & & & \multicolumn{2}{c}{\footnotesize{Out of Memory}} \\ 
% 789  & 5.9\%   & Union Square       & 9.3  & 3.9 & 9.2  & 4.4 & 5.98          & 2.01          & 6.54                 & 3.48        &4.68& 1.92        & 4.37                     & 1.85        \\
% 836  & 24.6\%  & Vienna Cathedral    & 8.2  & 1.2& 19.3  & 2.39 & 3.9  & 1.5           & 7.21                 & 2.83            &&     & 3.91                              & 1.1        \\
% 437  & 26.5\%  & Yorkminster         & 3.5  & 1.6& 4.5  & 1.6 & 2.52          & 0.99          & 2.47                 & 1.45       & 2.18& 0.92          & 2.27                    & 0.91       \\
% 2152 & 10.2\%  & Piccadilly          & 6.9  & 2.9& 22.0  & 9.7 & 4.75          & 1.91          & 3.93                 & 1.81        &2.44&0.58         & 3.63                    & 1.8         \\
% 332  & 29.3\% & NYC Library        & 3    & 1.3   & 3.9    & 1.5 & 1.9  
        %  & 1.18          & 2.63                 & 1.24       &&          & 1.75                    & 1.12  \\
% \hline    
% % \multicolumn{13}{c}{mn: mean of the angular error (in deg); md: median of the angular error (in deg);}                      \\
% \end{tabular}
% }
% \end{center}
% \vspace{-0.5em}
% \caption{Comparison of results on the \textit{\textbf{1DSfM}} dataset. We compare our method with various SOTA MRA methods. Mean(mn) and median(md) angular errors on the estimated absolute rotations are compared. The entries with the best performance are bolded.}
% \label{table:1dsfm_table}
% % \vspace{-1em}
% \end{table*}
% \begin{table}[!t]
%   \begin{center}
%      \scalebox{0.85}{
% \begin{tabular}{ccccccccc}
% \hline
%   & \multicolumn{4}{c}{Eval Dataset} &  \multicolumn{2}{c}{opt.} & \multicolumn{2}{c}{opt.}\\

% Robust. &  $|\mathcal{V}|$ & $|\mathcal{E}|$& $\sigma$ & $o$ &  mn & md  &  mn & md  \\
% \hline\hline
%  & $1000$ & $25\%$& $30^{\circ}$ & $15\%$ & 1.25 & 1.25 & 1.25 & 1.25 \\
%  & $1000$ & $25\%$& $30^{\circ}$ & $15\%$ & 1.25 & 1.25 & 1.25 & 1.25 \\
%  & $1000$ & $25\%$& $30^{\circ}$ & $15\%$ & 1.25 & 1.25 & 1.25 & 1.25 \\
%  & $1000$ & $25\%$& $30^{\circ}$ & $15\%$ & 1.25 & 1.25 & 1.25 & 1.25 \\
%  & $1000$ & $25\%$& $30^{\circ}$ & $15\%$ & 1.25 & 1.25 & 1.25 & 1.25 \\
%  & $1000$ & $25\%$& $30^{\circ}$ & $15\%$ & 1.25 & 1.25 & 1.25 & 1.25 \\
%  & $1000$ & $25\%$& $30^{\circ}$ & $15\%$ & 1.25 & 1.25 & 1.25 & 1.25 \\
%  & $1000$ & $25\%$& $30^{\circ}$ & $15\%$ & 1.25 & 1.25 & 1.25 & 1.25 \\
% \end{tabular}
% }
%   \end{center}
%   \caption{Comparison of results on the \textit{\textbf{1DSfM}} dataset. We compare our method with various SOTA MRA methods. Mean(mn) and median(md) angular errors on the estimated absolute rotations are compared. The entries with the best performance are bolded.}
% \label{table:robust_table}
% \end{table}

\begin{table}[!t]
  \begin{center}
     \scalebox{0.85}{
\begin{tabular}{cccccccc}
  \hline
  Robust. & Eval. & Train. & mn & md & Train. & mn & md & Time \\
  \hline
  \hline
  $|\mathcal{V}|$ & 300 & 300 & 1.22 & 1.22 & 600 & 1.22 & 1.22 \\
  $|\mathcal{V}|$ & 300 & 300 & 1.22 & 1.22 & 600 & 1.22 & 1.22 \\
  $|\mathcal{V}|$ & 300 & 300 & 1.22 & 1.22 & 600 & 1.22 & 1.22 \\
  \hline
  $|\mathcal{E}|$ & 300 & 300 & 1.22 & 1.22 & 600 & 1.22 & 1.22 \\
  $|\mathcal{E}|$ & 300 & 300 & 1.22 & 1.22 & 600 & 1.22 & 1.22 \\
  $|\mathcal{E}|$ & 300 & 300 & 1.22 & 1.22 & 600 & 1.22 & 1.22 \\
  \hline
  $|\mathcal{V}|$ & 300 & 300 & 1.22 & 1.22 & 600 & 1.22 & 1.22 \\
  $|\mathcal{V}|$ & 300 & 300 & 1.22 & 1.22 & 600 & 1.22 & 1.22 \\
  $|\mathcal{V}|$ & 300 & 300 & 1.22 & 1.22 & 600 & 1.22 & 1.22 \\
  \hline
  $|\mathcal{V}|$ & 300 & 300 & 1.22 & 1.22 & 600 & 1.22 & 1.22 \\
  $|\mathcal{V}|$ & 300 & 300 & 1.22 & 1.22 & 600 & 1.22 & 1.22 \\
  $|\mathcal{V}|$ & 300 & 300 & 1.22 & 1.22 & 600 & 1.22 & 1.22 \\
\end{tabular}
}
  \end{center}
  \caption{Comparison of results on the \textit{\textbf{1DSfM}} dataset. We compare our method with various SOTA MRA methods. Mean(mn) and median(md) angular errors on the estimated absolute rotations are compared. The entries with the best performance are bolded.}
\label{table:robust_table}
\end{table}

==> table/ablation_table.tex <==
% \begin{table*}[h!t]
% \begin{center}
% \scalebox{0.85}{
% \begin{tabular}{ccl|cc|cc|cc|cc|cc|cc}
% \hline
% \multicolumn{3}{c|}{Setting} & \multicolumn{2}{c|}{$t=1$} & \multicolumn{2}{c|}{$t=5$}& \multicolumn{2}{c|}{$t=20$} & \multicolumn{2}{c|}{$t=100$}& \multicolumn{2}{c|}{Avg. Time}& \multicolumn{2}{c}{CVPR2021} \\
% \hline \hline
% \#image & \#edge & Names & mn    & md    & mn    & md  & mn    & md  & mn   & md   & mn   & md& mn   & md   \\ 
%                   577  & 59.5\%  & Alamo               & 4.2  & 1.1  &6.2 &1.6 & 4.94          & 1.16          & 3.44                 & 1.16      & 2.82      &   0.88          & 2.89                      & 1.07                  \\
%     227  & 66.8\%  & Ellis Island       & 2.8  & 0.5& 3.9  & 1.2 & 2.59          & 0.64 & 2.61                 & 0.88           & 1.74&  0.46     & 1.88                   & 0.83                 \\
% 677  & 17.5\% & Gendarmenmarkt  & 37.6 & 7.7 & 41.6 & 13.3 & 4.51          & 2.94          & 44.9                 & 8.0     & 5.24 &     2.68           & 6.29  & 3.69  \\
% 341  & 30.7\%  & Madrid Metropolis              & 6.9  & 1.2 & 6.0  & 1.7 & 2.55 & 1.13          & 4.65                 & 1.26  &    3.05& 1.03               & 2.96                              & 1.09        \\
% 450  & 46.8\%  & Montreal Notre Dame & 1.5  & 0.5& 4.8  & 0.9 & 1.2           & 0.6           & 1.04        & 0.51       &0.86&0.46       & 0.91           & 0.5         \\
% 338  & 39.5\%  & Piazza del Popolo   & 4    & 0.8& 10.8    & 1.2 & 3.05          & 0.79          & 3.73                 & 1.93        &1.91&0.63         & 2.68                   & 0.76        \\
%   1084 & 10.9\%  & Roman Forum         & 3.1  & 1.5 & 13.2  & 8.2 & 2.39          & 1.31          & 2.62                 & 1.37     &2.55& 1.10           & 2.04                     & 1.19        \\
% 472  & 18.5\%  & Tower of London        & 3.9  & 2.4& 4.6  & 1.8 & 2.63          & 1.46          & 3.16                 & 2.2        &2.51&1.20          & 2.55                     & 1.25        \\
% 5058 & 4.6\%   & Trafalgar           & 3.5  & 2 & 48.6  & 13.2   & 5.33          & 2.25          &  \multicolumn{2}{c|}{-} & & & \multicolumn{2}{c}{\footnotesize{Out of Memory}} \\ 
% 789  & 5.9\%   & Union Square       & 9.3  & 3.9 & 9.2  & 4.4 & 5.98          & 2.01          & 6.54                 & 3.48        &4.68& 1.92        & 4.37                     & 1.85        \\
% 836  & 24.6\%  & Vienna Cathedral    & 8.2  & 1.2& 19.3  & 2.39 & 3.9  & 1.5           & 7.21                 & 2.83            &&     & 3.91                              & 1.1        \\
% 437  & 26.5\%  & Yorkminster         & 3.5  & 1.6& 4.5  & 1.6 & 2.52          & 0.99          & 2.47                 & 1.45       & 2.18& 0.92          & 2.27                    & 0.91       \\
% 2152 & 10.2\%  & Piccadilly          & 6.9  & 2.9& 22.0  & 9.7 & 4.75          & 1.91          & 3.93                 & 1.81        &2.44&0.58         & 3.63                    & 1.8         \\
% 332  & 29.3\% & NYC Library        & 3    & 1.3   & 3.9    & 1.5 & 1.9           & 1.18          & 2.63                 & 1.24       &&          & 1.75                    & 1.12  \\
% \hline    
% % \multicolumn{13}{c}{mn: mean of the angular error (in deg); md: median of the angular error (in deg);}                      \\
% \end{tabular}
% }
% \end{center}
% \vspace{-0.5em}
% \caption{Comparison of results on the \textit{\textbf{1DSfM}} dataset. We compare our method with various SOTA MRA methods. Mean(mn) and median(md) angular errors on the estimated absolute rotations are compared. The entries with the best performance are bolded.}
% \label{table:1dsfm_table}
% % \vspace{-1em}
% \end{table*}
\begin{table*}[h!t]
  \begin{center}


\begin{tabular}{cccccccclccccccccc}
\hline
  \multicolumn{4}{c}{Train Dataset}  & \multicolumn{4}{c}{Eval Dataset} & Method & \multicolumn{2}{c}{$t=1$} &\multicolumn{2}{c}{$t=5$} & \multicolumn{2}{c}{$t=20$}& \multicolumn{2}{c}{opt.} & Converge \\

$|\mathcal{V}|$ & $|\mathcal{E}|$& $\sigma$ & $o$ &  $|\mathcal{V}|$ & $|\mathcal{E}|$& $\sigma$ & $o$ & baseline & mn & md & mn & md & mn & md & mn & md & Y/N \\
\hline\hline
$|\mathcal{V}|$ & $|\mathcal{E}|$& $\sigma$ & $o$ &  $|\mathcal{V}|$ & $|\mathcal{E}|$& $\sigma$ & $o$ & baseline & mn & md & mn & md & mn & md & mn & md & Y/N \\
$|\mathcal{V}|$ & $|\mathcal{E}|$& $\sigma$ & $o$ &  $|\mathcal{V}|$ & $|\mathcal{E}|$& $\sigma$ & $o$ & baseline & mn & md & mn & md & mn & md & mn & md & Y/N \\
$|\mathcal{V}|$ & $|\mathcal{E}|$& $\sigma$ & $o$ &  $|\mathcal{V}|$ & $|\mathcal{E}|$& $\sigma$ & $o$ & baseline & mn & md & mn & md & mn & md & mn & md & Y/N \\
$|\mathcal{V}|$ & $|\mathcal{E}|$& $\sigma$ & $o$ &  $|\mathcal{V}|$ & $|\mathcal{E}|$& $\sigma$ & $o$ & baseline & mn & md & mn & md & mn & md & mn & md & Y/N \\
$|\mathcal{V}|$ & $|\mathcal{E}|$& $\sigma$ & $o$ &  $|\mathcal{V}|$ & $|\mathcal{E}|$& $\sigma$ & $o$ & baseline & mn & md & mn & md & mn & md & mn & md & Y/N \\
$|\mathcal{V}|$ & $|\mathcal{E}|$& $\sigma$ & $o$ &  $|\mathcal{V}|$ & $|\mathcal{E}|$& $\sigma$ & $o$ & baseline & mn & md & mn & md & mn & md & mn & md & Y/N \\
$|\mathcal{V}|$ & $|\mathcal{E}|$& $\sigma$ & $o$ &  $|\mathcal{V}|$ & $|\mathcal{E}|$& $\sigma$ & $o$ & baseline & mn & md & mn & md & mn & md & mn & md & Y/N \\
$|\mathcal{V}|$ & $|\mathcal{E}|$& $\sigma$ & $o$ &  $|\mathcal{V}|$ & $|\mathcal{E}|$& $\sigma$ & $o$ & baseline & mn & md & mn & md & mn & md & mn & md & Y/N \\
$|\mathcal{V}|$ & $|\mathcal{E}|$& $\sigma$ & $o$ &  $|\mathcal{V}|$ & $|\mathcal{E}|$& $\sigma$ & $o$ & baseline & mn & md & mn & md & mn & md & mn & md & Y/N \\
$|\mathcal{V}|$ & $|\mathcal{E}|$& $\sigma$ & $o$ &  $|\mathcal{V}|$ & $|\mathcal{E}|$& $\sigma$ & $o$ & baseline & mn & md & mn & md & mn & md & mn & md & Y/N \\
$|\mathcal{V}|$ & $|\mathcal{E}|$& $\sigma$ & $o$ &  $|\mathcal{V}|$ & $|\mathcal{E}|$& $\sigma$ & $o$ & baseline & mn & md & mn & md & mn & md & mn & md & Y/N \\
$|\mathcal{V}|$ & $|\mathcal{E}|$& $\sigma$ & $o$ &  $|\mathcal{V}|$ & $|\mathcal{E}|$& $\sigma$ & $o$ & baseline & mn & md & mn & md & mn & md & mn & md & Y/N \\
$|\mathcal{V}|$ & $|\mathcal{E}|$& $\sigma$ & $o$ &  $|\mathcal{V}|$ & $|\mathcal{E}|$& $\sigma$ & $o$ & baseline & mn & md & mn & md & mn & md & mn & md & Y/N \\
$|\mathcal{V}|$ & $|\mathcal{E}|$& $\sigma$ & $o$ &  $|\mathcal{V}|$ & $|\mathcal{E}|$& $\sigma$ & $o$ & baseline & mn & md & mn & md & mn & md & mn & md & Y/N \\
$|\mathcal{V}|$ & $|\mathcal{E}|$& $\sigma$ & $o$ &  $|\mathcal{V}|$ & $|\mathcal{E}|$& $\sigma$ & $o$ & baseline & mn & md & mn & md & mn & md & mn & md & Y/N \\
$|\mathcal{V}|$ & $|\mathcal{E}|$& $\sigma$ & $o$ &  $|\mathcal{V}|$ & $|\mathcal{E}|$& $\sigma$ & $o$ & baseline & mn & md & mn & md & mn & md & mn & md & Y/N \\
$|\mathcal{V}|$ & $|\mathcal{E}|$& $\sigma$ & $o$ &  $|\mathcal{V}|$ & $|\mathcal{E}|$& $\sigma$ & $o$ & baseline & mn & md & mn & md & mn & md & mn & md & Y/N \\
$|\mathcal{V}|$ & $|\mathcal{E}|$& $\sigma$ & $o$ &  $|\mathcal{V}|$ & $|\mathcal{E}|$& $\sigma$ & $o$ & baseline & mn & md & mn & md & mn & md & mn & md & Y/N \\
$|\mathcal{V}|$ & $|\mathcal{E}|$& $\sigma$ & $o$ &  $|\mathcal{V}|$ & $|\mathcal{E}|$& $\sigma$ & $o$ & baseline & mn & md & mn & md & mn & md & mn & md & Y/N \\

\end{tabular}

  \end{center}
  \caption{Comparison of results on the \textit{\textbf{1DSfM}} dataset. We compare our method with various SOTA MRA methods. Mean(mn) and median(md) angular errors on the estimated absolute rotations are compared. The entries with the best performance are bolded.}
\label{table:ablation_table}
\end{table*}

==> table/notation.tex <==
\begin{table}[!t]
\begin{center}
\scalebox{0.85}{
\begin{tabular}{c|c}
\hline
Symbol & Description \\
\hline \hline
$\mathbf{R}_{uv}$ & Observed relative orientation \\
$\check{\mathbf{R}}^{t}_{uv}$ & Rectified relative orientation at iter. $t$ \\
$\hat{\mathbf{R}}_{uv}|\bar{\mathbf{R}}_{uv}$ & Optimized $|$ Ground-Truth relative orientation\\
$\mathbf{R}_{u}$ & Initial absolute orientation \\
$\tilde{\mathbf{R}}^{t}_{u}|\tilde{\mathbf{R}}^{t}_{uv}$ & Estimated absolute $|$ relative orientation at iter. $t$\\
$\hat{\mathbf{R}}_{u}|\bar{\mathbf{R}}_{u}$ & Optimized $|$ Ground-Truth absolute orientation\\
$\mathcal{G}=(\mathcal{V}, \mathcal{E})$ & Graph $\mathcal{G}$ with node set $\mathcal{V}$ and edge set $\mathcal{E}$ \\
$\mathbf{f}_{u} | \mathbf{f}_{uv}$ & Feature on node $u$ $|$ edge $(u,v)$ \\
$\Theta(\mathbf{f}_{u}, \mathbf{f}_{uv}, \mathcal{G})$ & MPNN for graph $\mathcal{G}$ with $\mathbf{f}_{u}$ and $\mathbf{f}_{uv}$ \\
$\Phi$ &  multi-layered  linear  perceptions(MLP) \\
$d$ & Distance between two rotations \\
$C$ & Distance in feature space\\
$h^{t}$ & Hidden status at iter. $t$\\
$\mathcal{N}^{k}_{u}$ & $k$-order neighbor node set of node $u$\\
\hline    
% \multicolumn{13}{c}{mn: mean of the angular error (in deg); md: median of the angular error (in deg);}                      \\
\end{tabular}
}
\end{center}
\caption{The notations and symbols used in the manuscript \ping{you define way too many parameters. We need to significantly simplify your denotation to make it understandable. For example, $\mathbf{R}^*$ in Equation 1 and 2 are unnecessary. $\tilde{\mathbf{R}}$ in Equation 1 look also unnecessary. You can use $\mathbf{R}$ for both of them.} }
\vspace{-1em}
\label{table:notation}

% \vspace{-1em}
\end{table}


==> table/robust_table.tex <==
% \begin{table*}[h!t]
% \begin{center}
% \scalebox{0.85}{
% \begin{tabular}{ccl|cc|cc|cc|cc|cc|cc}
% \hline
% \multicolumn{3}{c|}{Setting} & \multicolumn{2}{c|}{$t=1$} & \multicolumn{2}{c|}{$t=5$}& \multicolumn{2}{c|}{$t=20$} & \multicolumn{2}{c|}{$t=100$}& \multicolumn{2}{c|}{Avg. Time}& \multicolumn{2}{c}{CVPR2021} \\
% \hline \hline
% \#image & \#edge & Names & mn    & md    & mn    & md  & mn    & md  & mn   & md   & mn   & md& mn   & md   \\ 
%                   577  & 59.5\%  & Alamo               & 4.2  & 1.1  &6.2 &1.6 & 4.94          & 1.16          & 3.44                 & 1.16      & 2.82      &   0.88          & 2.89                      & 1.07                  \\
%     227  & 66.8\%  & Ellis Island       & 2.8  & 0.5& 3.9  & 1.2 & 2.59          & 0.64 & 2.61                 & 0.88           & 1.74&  0.46     & 1.88                   & 0.83                 \\
% 677  & 17.5\% & Gendarmenmarkt  & 37.6 & 7.7 & 41.6 & 13.3 & 4.51          & 2.94          & 44.9                 & 8.0     & 5.24 &     2.68           & 6.29  & 3.69  \\
% 341  & 30.7\%  & Madrid Metropolis              & 6.9  & 1.2 & 6.0  & 1.7 & 2.55 & 1.13          & 4.65                 & 1.26  &    3.05& 1.03               & 2.96                              & 1.09        \\
% 450  & 46.8\%  & Montreal Notre Dame & 1.5  & 0.5& 4.8  & 0.9 & 1.2           & 0.6           & 1.04        & 0.51       &0.86&0.46       & 0.91           & 0.5         \\
% 338  & 39.5\%  & Piazza del Popolo   & 4    & 0.8& 10.8    & 1.2 & 3.05          & 0.79          & 3.73                 & 1.93        &1.91&0.63         & 2.68                   & 0.76        \\
%   1084 & 10.9\%  & Roman Forum         & 3.1  & 1.5 & 13.2  & 8.2 & 2.39          & 1.31          & 2.62                 & 1.37     &2.55& 1.10           & 2.04                     & 1.19        \\
% 472  & 18.5\%  & Tower of London        & 3.9  & 2.4& 4.6  & 1.8 & 2.63          & 1.46          & 3.16                 & 2.2        &2.51&1.20          & 2.55                     & 1.25        \\
% 5058 & 4.6\%   & Trafalgar           & 3.5  & 2 & 48.6  & 13.2   & 5.33          & 2.25          &  \multicolumn{2}{c|}{-} & & & \multicolumn{2}{c}{\footnotesize{Out of Memory}} \\ 
% 789  & 5.9\%   & Union Square       & 9.3  & 3.9 & 9.2  & 4.4 & 5.98          & 2.01          & 6.54                 & 3.48        &4.68& 1.92        & 4.37                     & 1.85        \\
% 836  & 24.6\%  & Vienna Cathedral    & 8.2  & 1.2& 19.3  & 2.39 & 3.9  & 1.5           & 7.21                 & 2.83            &&     & 3.91                              & 1.1        \\
% 437  & 26.5\%  & Yorkminster         & 3.5  & 1.6& 4.5  & 1.6 & 2.52          & 0.99          & 2.47                 & 1.45       & 2.18& 0.92          & 2.27                    & 0.91       \\
% 2152 & 10.2\%  & Piccadilly          & 6.9  & 2.9& 22.0  & 9.7 & 4.75          & 1.91          & 3.93                 & 1.81        &2.44&0.58         & 3.63                    & 1.8         \\
% 332  & 29.3\% & NYC Library        & 3    & 1.3   & 3.9    & 1.5 & 1.9           & 1.18          & 2.63                 & 1.24       &&          & 1.75                    & 1.12  \\
% \hline    
% % \multicolumn{13}{c}{mn: mean of the angular error (in deg); md: median of the angular error (in deg);}                      \\
% \end{tabular}
% }
% \end{center}
% \vspace{-0.5em}
% \caption{Comparison of results on the \textit{\textbf{1DSfM}} dataset. We compare our method with various SOTA MRA methods. Mean(mn) and median(md) angular errors on the estimated absolute rotations are compared. The entries with the best performance are bolded.}
% \label{table:1dsfm_table}
% % \vspace{-1em}
% \end{table*}
\begin{table*}[h!t]
  \begin{center}


\begin{tabular}{ccccccccccccc}
\hline
 & \multicolumn{4}{c}{Train Dataset}  & \multicolumn{4}{c}{Eval Dataset} &  \multicolumn{2}{c}{opt.} & \multicolumn{2}{c}{opt.}\\

robustness & $|\mathcal{V}|$ & $|\mathcal{E}|$& $\sigma$ & $o$ &  $|\mathcal{V}|$ & $|\mathcal{E}|$& $\sigma$ & $o$ &  mn & md  &  mn & md  \\
\hline\hline
node &$1000$ & $25\%$& $30^{\circ}$ & $15\%$ & $1000$ & $25\%$& $30^{\circ}$ & $15\%$ & 1.25 & 1.25 & 1.25 & 1.25 \\
node &$1000$ & $25\%$& $30^{\circ}$ & $15\%$ & $1000$ & $25\%$& $30^{\circ}$ & $15\%$ & 1.25 & 1.25 & 1.25 & 1.25 \\
node &$1000$ & $25\%$& $30^{\circ}$ & $15\%$ & $1000$ & $25\%$& $30^{\circ}$ & $15\%$ & 1.25 & 1.25 & 1.25 & 1.25 \\
node &$1000$ & $25\%$& $30^{\circ}$ & $15\%$ & $1000$ & $25\%$& $30^{\circ}$ & $15\%$ & 1.25 & 1.25 & 1.25 & 1.25 \\
node &$1000$ & $25\%$& $30^{\circ}$ & $15\%$ & $1000$ & $25\%$& $30^{\circ}$ & $15\%$ & 1.25 & 1.25 & 1.25 & 1.25 \\
node &$1000$ & $25\%$& $30^{\circ}$ & $15\%$ & $1000$ & $25\%$& $30^{\circ}$ & $15\%$ & 1.25 & 1.25 & 1.25 & 1.25 \\
node &$1000$ & $25\%$& $30^{\circ}$ & $15\%$ & $1000$ & $25\%$& $30^{\circ}$ & $15\%$ & 1.25 & 1.25 & 1.25 & 1.25 \\
node &$1000$ & $25\%$& $30^{\circ}$ & $15\%$ & $1000$ & $25\%$& $30^{\circ}$ & $15\%$ & 1.25 & 1.25 & 1.25 & 1.25 \\
\end{tabular}

  \end{center}
  \caption{Comparison of results on the \textit{\textbf{1DSfM}} dataset. We compare our method with various SOTA MRA methods. Mean(mn) and median(md) angular errors on the estimated absolute rotations are compared. The entries with the best performance are bolded.}
\label{table:robust_table}
\end{table*}
